Plasmonics enabled atomically thin linearly polarized emitter at room temperature

Two-dimensional transition metal di-chalcogenide semiconductors provide unique possibilities to investigate strongly confined excitonic physics and a plasmonic platform integrable to such materials constitutes a hybrid system that can be of interest to enable manipulation of their cumulative optical properties. Here we report tuning of excitonic emission from monolayer WSe2, mechanically exfoliated on top of a periodic two dimensional plasmonic array of elliptical gold (Au) nanodiscs. By exploiting the polarization-dependent nature of plasmonic resonance of the nano plasmonic array (NPA), the photoluminescence (PL) emission from the overlaid monolayer WSe2 could be significantly manipulated. PL is preferentially enhanced at the NPA covered regions of the ake when excited closer to the plasmonic resonant frequencies and previously unpolarized WSe2 PL emission gained ~ 20 up to 40 % degree of linear polarization at room temperature. Obtaining significant spectral overlap between the PL spectrum of WSe2 and the polarization tunable plasmonic resonance of the NPA plays a crucial role in this observation. The results demonstrate active tunability of optical emission from WSe2 by using an otherwise passive plasmonic environment and open the possibility of achieving atomically thin linearly polarized emitters at room temperature. In addition to fundamentally interesting physics of such interactions this can be highly desirable for ultrathin orientation sensitive opto-electronic device related applications.

==> mybib.tex <==
@article{srivastava2015QD,
  title={Optically active quantum dots in monolayer WSe2},
  author={Srivastava, Ajit and Sidler, Meinrad and Allain, Adrien V and Lembke, Dominik S and Kis, Andras and Imamo{\u{g}}lu, A},
  journal={Nature nanotechnology},
  volume={10},
  number={6},
  pages={491},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{potemski2015single,
  title={Single photon emitters in exfoliated WSe 2 structures},
  author={Koperski, M and Nogajewski, K and Arora, A and Cherkez, V and Mallet, P and Veuillen, J-Y and Marcus, J and Kossacki, P and Potemski, M},
  journal={Nature nanotechnology},
  volume={10},
  number={6},
  pages={503},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{he2015single,
  title={Single quantum emitters in monolayer semiconductors},
  author={He, Yu-Ming and Clark, Genevieve and Schaibley, John R and He, Yu and Chen, Ming-Cheng and Wei, Yu-Jia and Ding, Xing and Zhang, Qiang and Yao, Wang and Xu, Xiaodong and others},
  journal={Nature nanotechnology},
  volume={10},
  number={6},
  pages={497},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{potemski2016darktuning,
  title={Tuning valley polarization in a WSe 2 monolayer with a tiny magnetic field},
  author={Smole{\'n}ski, T and Goryca, M and Koperski, M and Faugeras, C and Kazimierczuk, T and Bogucki, A and Nogajewski, K and Kossacki, P and Potemski, M},
  journal={Physical Review X},
  volume={6},
  number={2},
  pages={021024},
  year={2016},
  publisher={APS}
}

@article{danovich2017dark,
  title={Dark trions and biexcitons in WS 2 and WSe 2 made bright by ee scattering},
  author={Danovich, Mark and Z{\'o}lyomi, Viktor and Fal’ko, Vladimir I},
  journal={Scientific Reports},
  volume={7},
  pages={45998},
  year={2017},
  publisher={Nature Publishing Group}
}

@article{heinz2015dark,
  title={Experimental evidence for dark excitons in monolayer WSe2},
  author={Zhang, Xiao-Xiao and You, Yumeng and Zhao, Shu Yang Frank and Heinz, Tony F},
  journal={Physical review letters},
  volume={115},
  number={25},
  pages={257403},
  year={2015},
  publisher={APS}
}
  
@article{urbaszek2014valley,
  title={Valley dynamics probed through charged and neutral exciton emission in monolayer WSe 2},
  author={Wang, G and Bouet, L and Lagarde, D and Vidal, M and Balocchi, A and Amand, T and Marie, X and Urbaszek, B},
  journal={Physical Review B},
  volume={90},
  number={7},
  pages={075413},
  year={2014},
  publisher={APS}
}
  
@article{urbaszek2015coherence,
  title={Double resonant Raman scattering and valley coherence generation in monolayer WSe 2},
  author={Wang, G and Glazov, MM and Robert, C and Amand, T and Marie, X and Urbaszek, B},
  journal={Physical review letters},
  volume={115},
  number={11},
  pages={117401},
  year={2015},
  publisher={APS}
}
@article{hao2016direct,
  title={Direct measurement of exciton valley coherence in monolayer WSe 2},
  author={Hao, Kai and Moody, Galan and Wu, Fengcheng and Dass, Chandriker Kavir and Xu, Lixiang and Chen, Chang-Hsiao and Sun, Liuyang and Li, Ming-Yang and Li, Lain-Jong and MacDonald, Allan H and others},
  journal={Nature Physics},
  volume={12},
  number={7},
  pages={677},
  year={2016},
  publisher={Nature Publishing Group}
}
@article{gonccalves2018plasmonexciton,
  title={Plasmon-exciton polaritons in two-dimensional semiconductor/metal interfaces},
  author={Gon{\c{c}}alves, PAD and Bertelsen, LP and Xiao, Sanshui and Mortensen, N Asger},
  journal={Physical Review B},
  volume={97},
  number={4},
  pages={041402},
  year={2018},
  publisher={APS}
}
@article{liu2015strong,
  title={Strong light--matter coupling in two-dimensional atomic crystals},
  author={Liu, Xiaoze and Galfsky, Tal and Sun, Zheng and Xia, Fengnian and Lin, Erh-chen and Lee, Yi-Hsien and K{\'e}na-Cohen, St{\'e}phane and Menon, Vinod M},
  journal={Nature Photonics},
  volume={9},
  number={1},
  pages={30},
  year={2015},
  publisher={Nature Publishing Group}
}
  
@article{dufferwiel2015,
  title={Exciton--polaritons in van der Waals heterostructures embedded in tunable microcavities},
  author={Dufferwiel, S and Schwarz, S and Withers, F and Trichet, AAP and Li, F and Sich, M and Del Pozo-Zamudio, O and Clark, C and Nalitov, A and Solnyshkov, DD and others},
  journal={Nature communications},
  volume={6},
  pages={8579},
  year={2015},
  publisher={Nature Publishing Group}
}

@article{schneider2018,
  title={Two-dimensional semiconductors in the regime of strong light-matter coupling},
  author={Schneider, Christian and Glazov, Mikhail M and Korn, Tobias and H{\"o}fling, Sven and Urbaszek, Bernhard},
  journal={Nature communications},
  volume={9},
  number={1},
  pages={2695},
  year={2018},
  publisher={Nature Publishing Group}
}

@article{schaibley2016valleytronics,
  title={Valleytronics in 2D materials},
  author={Schaibley, John R and Yu, Hongyi and Clark, Genevieve and Rivera, Pasqual and Ross, Jason S and Seyler, Kyle L and Yao, Wang and Xu, Xiaodong},
  journal={Nature Reviews Materials},
  volume={1},
  number={11},
  pages={16055},
  year={2016},
  publisher={Nature Publishing Group}
}
@article{wang2012electronics,
  title={Electronics and optoelectronics of two-dimensional transition metal dichalcogenides},
  author={Wang, Qing Hua and Kalantar-Zadeh, Kourosh and Kis, Andras and Coleman, Jonathan N and Strano, Michael S},
  journal={Nature nanotechnology},
  volume={7},
  number={11},
  pages={699},
  year={2012},
  publisher={Nature Publishing Group}
}
@article{wangreview,
  title = {Colloquium: Excitons in atomically thin transition metal dichalcogenides},
  author = {Wang, Gang and Chernikov, Alexey and Glazov, Mikhail M. and Heinz, Tony F. and Marie, Xavier and Amand, Thierry and Urbaszek, Bernhard},
  journal = {Rev. Mod. Phys.},
  volume = {90},
  issue = {2},
  pages = {021001},
  numpages = {25},
  year = {2018},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.90.021001},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.90.021001}
}
  
@article{agarwal2018arxiv,
  title={Observation and active control of a collective polariton mode and polaritonic band gap in few-layer WS2 strongly coupled with plasmonic lattices},
  author={Liu, Wenjing and Wang, Yuhui and Zheng, Biyuan and Hwang, Minsoo and Ji, Zhurun and Liu, Gerui and Li, Ziwei and Sorger, Volker J and Pan, Anlian and Agarwal, Ritesh},
  journal={arXiv preprint arXiv:1808.06554},
  year={2018}
}
  
@article{agarwal2017,
  title={Understanding the Different Exciton--Plasmon Coupling Regimes in Two-Dimensional Semiconductors Coupled with Plasmonic Lattices: A Combined Experimental and Unified Equation of Motion Approach},
  author={Liu, Wenjing and Wang, Yuhui and Naylor, Carl H and Lee, Bumsu and Zheng, Biyuan and Liu, Gerui and Johnson, AT Charlie and Pan, Anlian and Agarwal, Ritesh},
  journal={ACS Photonics},
  volume={5},
  number={1},
  pages={192--204},
  year={2017},
  publisher={ACS Publications}
}
  
@article{agarwal2017a,
  title={Electrical tuning of exciton--plasmon polariton coupling in monolayer MoS2 integrated with plasmonic nanoantenna lattice},
  author={Lee, Bumsu and Liu, Wenjing and Naylor, Carl H and Park, Joohee and Malek, Stephanie C and Berger, Jacob S and Johnson, AT Charlie and Agarwal, Ritesh},
  journal={Nano letters},
  volume={17},
  number={7},
  pages={4541--4547},
  year={2017},
  publisher={ACS Publications}
}
  
@article{agarwal2016strong,
title={Strong exciton--plasmon coupling in MoS2 coupled with plasmonic lattice},
author={Liu, Wenjing and Lee, Bumsu and Naylor, Carl H and Ee, Ho-Seok and Park, Joohee and Johnson, AT Charlie and Agarwal, Ritesh},
  journal={Nano letters},
  volume={16},
  number={2},
  pages={1262--1269},
  year={2016},
  publisher={ACS Publications}
}
  
 @article{agarwal2015fano,
  title={Fano resonance and spectrally modified photoluminescence enhancement in monolayer MoS2 integrated with plasmonic nanoantenna array},
  author={Lee, Bumsu and Park, Joohee and Han, Gang Hee and Ee, Ho-Seok and Naylor, Carl H and Liu, Wenjing and Johnson, AT Charlie and Agarwal, Ritesh},
  journal={Nano letters},
  volume={15},
  number={5},
  pages={3646--3653},
  year={2015},
  publisher={ACS Publications}
}
  
@article{blauth2018coupling,
title={Coupling Single Photons from Discrete Quantum Emitters in WSe2 to Lithographically Defined Plasmonic Slot Waveguides},
author={Blauth, M{\"a}x and Juergensen, M and Vest, Gwena{\"e}lle and Hartwig, Oliver and Prechtl, Maximilian and Cerne, John and Finley, Jonathan J and Kaniber, Michael},
journal={Nano letters},
volume={18},
number={11},
pages={6812--6819},
year={2018},
publisher={ACS Publications}
}



@article{biswanath,
  title={Control of Strong Light--Matter Interaction in Monolayer WS2 through Electric Field Gating},
  author={Chakraborty, Biswanath and Gu, Jie and Sun, Zheng and Khatoniar, Mandeep and Bushati, Rezlind and Boehmke, Alexandra L and Koots, Rian and Menon, Vinod M},
  journal={Nano letters},
  volume={18},
  number={10},
  pages={6455--6460},
  year={2018},
  publisher={ACS Publications}
}

@article{heinz,
  title = {Atomically Thin ${\mathrm{MoS}}_{2}$: A New Direct-Gap Semiconductor},
  author = {Mak, Kin Fai and Lee, Changgu and Hone, James and Shan, Jie and Heinz, Tony F.},
  journal = {Phys. Rev. Lett.},
  volume = {105},
  issue = {13},
  pages = {136805},
  numpages = {4},
  year = {2010},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.105.136805},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.105.136805}
}

@article{splendiani,
  title={Emerging photoluminescence in monolayer MoS2},
  author={Splendiani, Andrea and Sun, Liang and Zhang, Yuanbo and Li, Tianshu and Kim, Jonghwan and Chim, Chi-Yung and Galli, Giulia and Wang, Feng},
  journal={Nano letters},
  volume={10},
  number={4},
  pages={1271--1275},
  year={2010},
  publisher={ACS Publications}
}

@article{lamprecht,
  title = {Metal Nanoparticle Gratings: Influence of Dipolar Particle Interaction on the Plasmon Resonance},
  author = {Lamprecht, B. and Schider, G. and Lechner, R. T. and Ditlbacher, H. and Krenn, J. R. and Leitner, A. and Aussenegg, F. R.},
  journal = {Phys. Rev. Lett.},
  volume = {84},
  issue = {20},
  pages = {4721--4724},
  numpages = {0},
  year = {2000},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.84.4721},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.84.4721}
}


@article{Meier,
author = {M. Meier and A. Wokaun and P. F. Liao},
journal = {J. Opt. Soc. Am. B},
keywords = {Evanescent waves; Light scattering; Mie theory; Power spectral density; Raman scattering; Spatial frequency},
number = {6},
pages = {931--949},
publisher = {OSA},
title = {Enhanced fields on rough surfaces: dipolar interactions among particles of sizes exceeding the Rayleigh limit},
volume = {2},
year = {1985},
url = {http://josab.osa.org/abstract.cfm?URI=josab-2-6-931},
doi = {10.1364/JOSAB.2.000931},
}

@Article{Butler,
author = {Butler, Sheneve Z. and Hollen, Shawna M. and Cao, Linyou and Cui, Yi and Gupta, Jay A. and Gutiérrez, Humberto R. and Heinz, Tony F. and Hong, Seung Sae and Huang, Jiaxing and Ismach, Ariel F. and Johnston-Halperin, Ezekiel and Kuno, Masaru and Plashnitsa, Vladimir V. and Robinson, Richard D. and Ruoff, Rodney S. and Salahuddin, Sayeef and Shan, Jie and Shi, Li and Spencer, Michael G. and Terrones, Mauricio and Windl, Wolfgang and Goldberger, Joshua E.},
title = {Progress, Challenges, and Opportunities in Two-Dimensional Materials Beyond Graphene},
journal = {ACS Nano},
volume = {7},
number = {4},
pages = {2898-2926},
year = {2013},
doi = {10.1021/nn400280c},
note ={PMID: 23464873},
URL = { 
       https://doi.org/10.1021/nn400280c
},
eprint = { 
       https://doi.org/10.1021/nn400280c},
    
}


@article{Ding,
author = {Ding, Yufeng and Wei, Chengrong and Su, Huimin and Sun, Shuoyan and Tang, Zhiyong and Wang, Zhaona and Li, Guixin and Liu, Dahe and Gwo, Shangjr and Dai, Junfeng and Shi, Jinwei},
title = {Second Harmonic Generation Covering the Entire Visible Range from a 2D Material–Plasmon Hybrid Metasurface},
journal = {Advanced Optical Materials},
volume = {9},
number = {16},
pages = {2100625},
year = {2021},
doi = {https://doi.org/10.1002/adom.202100625},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/adom.202100625},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/adom.202100625},

}

@article{Carlson,
 author = {Carlson, Chelsea and Salzwedel, Robert and Selig, Malte and Knorr, Andreas and Hughes, Stephen},
title = {Strong coupling regime and hybrid quasinormal modes from a single plasmonic resonator coupled to a transition metal dichalcogenide monolayer},
 journal = {Phys. Rev. B},
 volume = {104},
  issue = {12},
  pages = {125424},
  numpages = {13},
 year = {2021},
 month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.104.125424},
 url = {https://link.aps.org/doi/10.1103/PhysRevB.104.125424},
}


}



